A linear MARS method for three-dimensional interface tracking

For explicit interface tracking in three dimensions, we propose a linear MARS method that (a) represents the interface by a partially ordered set of glued surfaces and approximates each glued surface with a triangular mesh, (b) maintains an $(r,h,\theta)$-regularity on each triangular mesh so that the distance between any pair of adjacent markers is within the range $[rh,h]$ and no angle in any triangle is less than $\theta$, (c) applies to three-dimensional continua with arbitrarily complex topology and geometry, (d) preserves topological structures and geometric features of moving phases under diffeomorphic and isometric flow maps, and (e) achieves second-order and third-order accuracy in terms of the Lagrangian and Eulerian length scales, respectively. Results of classic benchmark tests verify the effectiveness of the novel mesh adjustment algorithms in enforcing the $(r,h,\theta)$-regularity and demonstrate the high accuracy and efficiency of the proposed linear MARS method.

==> tab/deform.tex <==
 \begin{tabular}{c|ccccccc}
     \hline \hline
%    \multicolumn{2}{c|}{\rule[-3mm]{0mm}{8mm} Methods }
     methods
     & $h=\frac{1}{32}$ & rate & $h=\frac{1}{64}$ & rate &  $h=\frac{1}{128}$
     & rate &  $h=\frac{1}{256}$\\
     \hline 
   linearMARS ($h_{L} = 0.5h$)
     &  6.24e-4 &       2.04 &   1.52e-4 & 2.00 &   3.78e-5 & 1.99&
  9.52e-6\\
   linearMARS ($h_{L} = 6h^{\frac{3}{2}}$)
     &  2.49e-3 &       2.96 & 3.20e-4 &       3.01 &   3.96e-5 &3.01&
  4.93e-6\\
     \hline \hline
   \end{tabular}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: t
%%% End:

